Public Evidence from Secret Ballots

Elections seem simple---aren't they just counting? But they have a unique, challenging combination of security and privacy requirements. The stakes are high; the context is adversarial; the electorate needs to be convinced that the results are correct; and the secrecy of the ballot must be ensured. And they have practical constraints: time is of the essence, and voting systems need to be affordable and maintainable, and usable by voters, election officials, and pollworkers. It is thus not surprising that voting is a rich research area spanning theory, applied cryptography, practical systems analysis, usable security, and statistics. Election integrity involves two key concepts: convincing evidence that outcomes are correct and privacy, which amounts to convincing assurance that there is no evidence about how any given person voted. These are obviously in tension. We examine how current systems walk this tightrope.

==> BallotCastingAssurance.tex <==
\medskip
\subsubsection{Ballot Casting Assurance}

%Most cast-as-intended verification protocols rely on human procedures and hence have
%a non-negligible soundness error.  
The notion of {\em ballot casting assurance\/} (first introduced in \cite{Adida-Neff})
is a measure of the confidence a voter can have that a vote has been cast as intended.
We offer a drastically different definition to quantify the level of assurance.

\begin{definition}
An election system is said to have {\bf ballot casting assurance\/} $\gamma$
%if, after voting, a rational voter has confidence that with probability at least $\gamma$,
%her intended selections were correctly cast.  
%if the casting of an unintended
%vote is detected with probability at least $\gamma$.
if there exists a strategy for the voter
guaranteeing that for any adversarial strategy
the voter is able to cast a vote exactly as intended
(or catch the voting system cheating)
with probability at least $1 - \gamma$.
\end{definition}

The value of $\gamma$ is a probability in the range $0\le\gamma\le1$,
and this value may be parameterized by both system settings and voter actions.
For instance, a system which uses an $r$-round interactive proof in which each
round independently has a 50\% probability of revealing an incorrect casting,
then the ballot casting assurance is $\gamma=1-1/2^r$



%(Note that most individual voters will likely not choose to spoil any ballots
%and will therefore individually have ballot casting assurance of $\gamma=0$.
%However, as long as a malicious system cannot predict which voters will spoil ballots,
%the overall confidence in the integrity of an election can be quite high.)

\OpenProblems{
\begin{itemize}

\item Is there a good way to measure the casting assurance of an entire election?

\item Are there other measures that better capture voter confidence?

\end{itemize}
}



==> ProblemSpace.tex <==
\red{VT: shifted all but these 4 para's into intro.}


Many election systems act by anonymizing ballots and then revealing
their contents.  However, this too can impact privacy.  Write-ins can
be used to reveal ones identity to a coercer: ``Vote for me as mayor
and write in your own name for dog-catcher.''  Even if write-ins are
not allowed, {\em pattern voting\/} can reveal identity in a ballot
with many races: ``Mark your full ballot in precisely this way
including this unique pattern of votes on lesser contests.''  While
contest-splitting (segmenting each ballot to effectively create
separate elections for each contest) can address some of these
concerns, it can add complexity for voters and doesn't solve some
related problems.

The {\em Italian attack\/} is named for a practice that was once
prevalent in Sicily.  A municipal council (of say ten members) would
be elected by instructing voters to list the names of the people they
supported.  The elected council would consist of those people whose
names appeared on the most ballots.  Prior to each election, local
bosses would assign a distinct permutation of their preferred names to
each voter.  If your assigned permutation was not on one of the
ballots counted, you would face the consequences.

A similar privacy compromise can be seen in elections which support
preferential voting.  Some recent Australian elections have had more
than fifty candidates which voters were required to rank.  The order
of the least preferred candidates could be used as a unique identifier
to reveal the identity of a voter.

Even if we exclude privacy compromises which take place through the
release of public data, there are other privacy risks which must be
managed.  If voters achieve privacy by encrypting their selections,
the holders of decryption keys can (perhaps in collusion) view their
votes.  If voters make their selections on devices out of their
immediate control (perhaps, official election equipment), then it is
difficult to assure them that these devices are not retaining
information that could later compromise their privacy.  If voters make
their selections on their own devices, then there is an even greater
risk that these devices could be infected with malware that records
(and perhaps even alters) their selections.


==> Terminology.tex <==
\newpage
\appendix{Terminology}

Convention: we're going to use
\begin{itemize}
\item{\bf social choice function}  the mathematical function mapping vote profiles to election outcomes, {\it e.g.} Condorcet, IRV, Schulze,
\item{\bf voting system specification} 
for the process and protocol description, the protocol and process description {\it e.g.} STAR as designed, PaV, Opscan+RLA,
\item{\bf voting system implementation} code, etc {\it e.g.} iVote, vVote, STAR when implemented.
\end{itemize}


==> ThreatsAndThreatModels.tex <==
\section{Threats and Threat Models}
\label{subsec:threats}

%\epigraph{As long as I count the votes, what are you going to do about it?}{\textit{William Marcy Tweed}}

In order to understand the security of diverse voting systems, we
begin by laying out a threat model that considers a generalized voting
system.  Who the adversaries are, what motivates them and how effectively they can
attack systems are critical
questions.
Our model is largely inspired by the work of the California Top-to-Bottom Review~\cite{California-TTBR-site}.

\medskip
\subsubsection*{Adversary Goals}

Election attackers typically act out of political motivation, with the goal of electing their
preferred candidate or policy, or rejecting candidates and policies they do not like. Swaying
election results can take place at many junctures in the election process, at varying scale. Attackers
corrupt election results in three major ways: {\em{removing ballots}} in order to disenfranchise certain
groups of voters or all voters, {\em{adding or manipulating ballots}} to overshadow or change results
from valid ballots, and {\em{coercing voters}} to discourage voters from voting or to change the
ballots that they cast.

In order to achieve these results, adversaries can destroy or alter election evidence,  alter
conditions in precincts to make voting infeasible, or prevent correct tabulation of results. Attackers can
corrupt voting machines to change or discard voter's intended choices. Attackers
can coerce voters by buying votes, dissuade them from voting, or otherwise threaten voters who do not
vote the attacker's preference if voters' privacy is compromised. These methods require
varying degrees of sophistication, coordination, and infiltration of election processes.

\medskip
\subsubsection*{Who are the Adversaries?}
\label{sec:adversaries}

Adversaries are
differentiated by the level of access they have to the election and the election process.
Insiders include election officials and voting technology vendor employees, but also less obvious insiders such
as janitors, couriers, and suppliers of hardware or of other software running on the voting machines. Adversaries
in these positions can compromise election integrity in numerous ways, and moreover can perpetrate
attacks at a much greater scale.
Malicious poll workers also fall into the insider group, however the scale at which they can affect
elections is generally restricted to affecting votes at a per-precinct or per-machine basis.
Voters themselves might also be attackers.

\medskip
\subsubsection*{Types of Attacks}
\label{sec:attack-types}

Attacks can be classified along many dimensions. An important factor for classifying attacks is
\emph{detectability}: some attacks, like ballot destruction, are relatively detectable, while others,
like coercion, are not. Some attacks are \emph{recoverable}, meaning that an election can continue
despite the compromise, while others are not. For instance, the destruction of a voting machine is
recoverable, as prompt replacement of the machine will prevent voters from being disenfranchised.
Widespread coercion or the destruction of ballots, however, are not recoverable, as valid election
results cannot be determined or reconstructed.


==> Traditional.tex <==
\section{``Traditional'' Voting Systems}
\label{sec:traditional}

Below we examine a variety of voting systems as they have been used in the
United States and elsewhere up to the present day. None of these systems fully
satisfy the properties of end-to-end verifiability, but nevertheless do have
some redeeming qualities that will better inform our discussion.

\medskip % DO NOT REMOVE
\subsection{Hand-marked paper ballots}
We first consider the hand-marked paper ballot. In modern
secret-ballot designs, voters are given blank sheets and will
use pen or pencil to indicate their selections.

%% Designs vary worldwide. In some elections where only one or two issues
%% are being voted, they might have separate ballot papers and
%% separate ballot boxes for each issue. Of course, this
%% sort of design doesn't scale when there are as many as 100 different
%% issues (common in some U.S. states) or when the voter is being asked
%% to, albeit optionally, specify a total ordering over as many as 100 different
%% candidates (Australia, others).
%%
%% Also, the standards for interpreting hand-marked paper ballots vary
%% widely. Some states define a legal standard of whether the ``intent of
%% the voter'' can be discerned, while other states have far more
%% specific standards, for example concerning a minimum percentage of an
%% oval being filled by the voter's mark. These issues notably came to a
%% head in the very close 2008 Minnesota U.S. Senate race between Franken and
%% Coleman. (Minnesota Public Radio has placed many of the disputed ballot images
%% online, allowing its viewers to offer up their own interpretations~\cite{mpr-ambiguous-ballots2008}.)

Hand-marked ballots may be manually tallied, or they may be machine tallied
through one of two processes, named for where the scanning machinery is
located: {\em precinct-count optical scan} (PCOS) vs. {\em central-count
optical scan}. In the former case, the scanner is mounted to the top of the
ballot box, giving it the ability to not only compute a local tally, but also
to reject malformed ballots. Typically, this means rejecting \emph{overvotes},
where a voter has indicated more than one selection in a race where they are
only allowed to specify a single candidate. The voter can see that his or her
ballot has been rejected, and can try to vote again, correctly. In the case of
central-count optical scan, the voter is gone and overvoted ballots must be
ignored, at least for the races in which they have overvoted.

%% PCOS is sometimes combined with {\em ballot-on-demand} printing, as used for
%% {\em early voting centers} or {\em election-day vote centers}, where voters are
%% no longer required to go to their specific home precinct. Instead, any of
%% potentially thousands of distinct ballot styles must be supported. Using laser
%% printers, each voter gets their proper ballot, with barcodes or other indicia
%% representing a ballot style identifier.  Vote centers fundamentally require
%% electronic tallying of ballots, since there may well be a single voter, of a
%% given ballot style, who presents themselves to vote at a given vote center. Any
%% manual tallying process would compromise that voter's anonymity.

Because of their fundamental lack of software (except in tallying devices),
these ballots are inherently software independent. Additionally, well-mixed
paper ballots achieve everlasting privacy, as it is impossible to associate the
identity of a voter with their ballot (except in perverse cases, such as a
write-in vote indicating the voter's name). The in-person voting allows for
coercion resistance (as discussed in Section~\ref{sec:CR})
and paper ballots are verifiably cast-as-intended assuming the voters carefully
check their markings on the hand-counted or optical-scan ballot. Due to their
physical nature, paper ballots are also easily audited, making them verifiably
counted-as-collected.

\subsection{Vote-by-mail}
\label{sec:vbm}
Paper ballots are also used widely for {\em postal voting}, where
blank ballots are mailed to registered voters, who fill them out at home and
then mail them back, often in special envelopes that allow the voter's identity
and signature to be validated, after which the ballot can be extracted and
processed anonymously through what otherwise appears to be a normal
central-count optical scan system.

Postal ballots retain most of the qualities associated with standard paper
ballots, but they do not offer coercion resistance (see
Section~\ref{sec:CR}).


%% Paper ballots, of all sorts, have a variety of beneficial properties
%% that guarantee they'll continue to be widely used, well into the
%% future.

%% \begin{itemize}
%% \item Cost: Paper is relatively cheap.
%% \item Scalability: Tables, desks, and pens are readily available,
%%   even in a makeshift fashion,
%%   allowing higher volumes of voters to be supported
%%   without a commensurate increase in equipment costs.
%% \item Usability: We have a population that is familiar with paper
%%   forms. Filling in a bubble with a pen is a task for which they've
%%   already been trained. In countries with low literacy levels, paper
%%   ballots are typically augmented with imagery and colors for each
%%   candidate or political party. That said,
%%   paper ballots are fundamentally challenging to operate without
%%   assistance for voters with zero vision, low motor control, or many other
%%   issues. In many areas, DRE devices (see below) are used to augment
%%   paper ballots for precisely these populations.
%% \item Auditability: Even when paper ballots are tabulated
%%   electronically, they can be sampled and compared to the electronic
%%   records (see Section~\ref{sec:Statistics}).
%% \end{itemize}

\medskip % DO NOT REMOVE
\subsection{Direct Recording Electronic voting systems (DREs)}
\label{sec:dre}
%% Prior to 2000, the market share for electronic voting systems was
%% minuscule. This changed in 2002 after the U.S. Congress allocated billions of
%% dollars to replace failed punchcard and mechanical lever machines.

%% We will discuss the security properties of the systems below, but
%% first it's worthwhile to present a basic taxonomy of these systems and
%% understand the claimed benefits they offered over their predecessors.

DRE voting systems eliminate all paper from
the process of casting a ballot. Voters are authorized to cast a ballot, they
go through a form-filling process to specify their intent, and then they
indicate their completion of the task. The specifics vary across each system.
For example, Diebold systems~\cite{hursti06diebold,feldman07diebold} use smartcards to
authorize machines and indicate ballot styles, while Hart InterCivic
systems~\cite{California-TTBR-site} use a local network in the polling place,
allowing a ``controller'' device to send authorization messages to machines and
collect cast ballots when the voter is finished. These systems were popularized
due to their fast tabulation of results and extensible accessibility features to
allow a broader population of voters to vote regardless of physical ability.
DREs also allow for easy ballot management, since any changes are purely made
in software and ballots do not have to be reprinted if an error is made. DREs
also notify voters of overvoting (and undervoting) inline, ostensibly lowering
voter error rates (though this tends to be
overstated~\cite{everett08chi-dre-usability}).

However, as there was little effort put into DRE design regarding verifiability,
these machines are severely lacking in security properties and do not even
retain the properties of simple paper. Not only is there no recourse if a DRE
fails during an election (either maliciously or not), but there is rarely even
a way to tell if failure has occurred, both on the part of the voters and the
election officials. DREs have been shown to have many
vulnerabilities~\cite{EVERESTmain,California-TTBR-site,feldman07diebold,wallach2006security}.
In fact, the only security property under our analysis that DREs provide is coercion
resistance, since they are deployed as in-person voting systems and---assuming
they are designed correctly and not tampered with---they generate
no evidence that a voter could use to reveal their vote.

%% \begin{itemize}
%% \item Rapid tallying: Who won? Tell us now! Electronic results are
%%   fundamentally easier and faster to tally. Some DRE systems included
%%   the use of modems to transmit results from polling places via analog
%%   modems.
%% \item Accessibility features: Because a voting machine is fundamentally
%%   a general-purpose computer, it can display text in any language (for
%%   voters for whom English is not their primary language), rendering
%%   the text in larger and/or higher contrast text (for low-vision
%%   voters), augmented by audio output (to help
%%   low-vision and zero-vision voters, as well as illiterate and
%%   dyslexic voters), and specialized input devices (to help low motor-control
%%   voters), allowing a much broader population to cast
%%   ballots without external assistance.
%% \item Ballot flexibility: One of the concerns with earlier mechanical
%%   lever machines and punchcard systems was that newer ballots were
%%   getting too big: too many races/issues and too many candidates to
%%   fit in some races. DREs brought the promise of handling such ballots
%%   with ease. They also fit nicely into vote centers, handling
%%   thousands of ballot styles.
%% \item Improved error handling: While PCOS systems can reject ballots
%%   for being overvoted, they still allow undervoted ballots. A DRE
%%   system can be configured to warn voters who undervote, and it can
%%   completely eliminate overvoting (e.g., by implementing ``radio
%%   button'' selection policies). (Usability experiments later showed that
%%   these benefits were overstated~\cite{everett08chi-dre-usability}.)
%% \item Faster recounts and audits: When all of the election records are
%%   electronic, then they're not only faster to tally, they're also
%%   faster to recount. In some states' recount procedures, electronic
%%   records would be printed on paper then tallied manually. Individual
%%   machines typically have their own records of the votes cast on them.
%%   These records have also been manually extracted and tabulated as
%%   part of some recount procedures. Vendors have also made claims to
%%   verify the integrity of the code on the voting machines as part of
%%   their recounting/auditing procedures.
%% \end{itemize}

%% Unfortunately, these vendors made security claims that
%% turned out to be wildly exaggerated; see Section~\ref{subsec:realworld}.

\subsection{Voter-verified paper audit trail (VVPAT)}
In the mid 2000s,
most DRE vendors offered VVPAT attachments as a means of compensating
for the lack of verifiability.  The VVPAT would allow the voter to see a printout
of their ballot selections before finalizing their vote, providing an
opportunity to verify a {\em tangible
record} for accuracy. Most commonly, VVPAT printers used {\em
continuous thermal paper rolls}, visible to the voter through a plastic window.
Implemented correctly, a VVPAT can offer DREs software independence, as there is
now auditable evidence from an election that is decoupled from the software.
Apart from this, however, DREs with VVPAT still suffer the same inadequacies as
DREs without.
%% TODO: Reference Rebecca Mercuri's work here

\subsection{Analysis of Real-World Pollsite Systems}
\label{subsec:realworld}

Security researchers have managed to study many different voting
systems that have been widely deployed in real-world elections.  Since
election authorities and vendors sometimes do not welcome such
scrutiny, a recurring challenge has been to obtain the necessary
access to voting machines or server systems. In virtually every case
where a widely fielded computer voting system has been subjected to
rigorous security scrutiny, researchers have found serious
vulnerabilities with the potential to violate the integrity and
privacy requirements.

The first e-voting system to receive significant academic scrutiny was the
Diebold AccuVote-TS, the most widely deployed e-voting platform in the
U.S. during the mid-2000s~\cite{EDS06}.  A prototypical DRE, it was
based on Windows CE, interacted with the user via an integrated
touchscreen LCD, and used a removable memory card to input ballot
definitions and offload results~\cite{feldman07diebold}.  Kohno
et~al. examined a leaked version of the source code\footnote{Diebold
  employees had stored a copy of the code on a company FTP site that
  was accessible to the public, where it was discovered by Bev Harris
  of BlackBoxVoting~\cite{jones03ftp}.} in 2003 and found many design
errors and vulnerabilities~\cite{kohno03voting}, which Diebold
dismissed as ``unrealistic''~\cite{DESTR03}.  In 2007, Feldman
et~al.\@ obtained an AccuVote-TS from an anonymous private party; they
confirmed the earlier vulnerabilities and showed that all records
of the vote were under the control of user-space
software~\cite{feldman07diebold}.  They also developed a \emph{voting
  machine virus} that would spread vote-stealing code
automatically via the removable memory cards during normal pre- and
post-election activities by exploited an unauthenticated software
update mechanism.

Following these and other early
studies~\cite{COMPU03,SAIC03,RABA04,hursti06diebold,ftt06minibar}, two
states commissioned comprehensive security reviews of their election
technology.  In 2007, California Secretary of State State Debra Bowen
conducted a ``top-to-bottom review''
(TTBR)~\cite{California-TTBR-site}, that examined systems manufactured
by Hart InterCivic, Sequoia Voting Systems, and Premier Election
Systems (formerly Diebold).  The state compelled the vendors to make
their code available for the evaluation.  David Wagner of
U.C.~Berkeley led a 40-person team that performed source code review
and red team testing.  They discovered numerous problems in all three
vendors' systems, including exploitable buffer overflows and
ineffective cryptography, such as hard-coded keys.  These problems
could allow vote-stealing code to spread virally via the election
management systems and allow election workers to compromise voters'
privacy.  The same year, Ohio initiated a similar study, Project
\textsc{EVEREST}~\cite{EVERESTmain}, that examined systems from ES\&S, Hart
InterCivic, and Premier.  Remarkably, although Ohio studied the same
Diebold and Sequoia systems as California, the team found yet more
vulnerabilities that had been overlooked in earlier analyses.

These DRE systems were quite complex: each used several hundred
thousand lines of code. In contrast, India, the world's largest
democracy, uses DREs nationwide, based on a very simple embedded
system design with no reprogrammable software and only switches and
LEDs for input and output.  In 2010, researchers reverse engineered an
India DRE provided by an anonymous whistle blower~\cite{india-ccs10} and showed
showed that their simplicity makes them susceptible to low-cost
hardware tampering attacks that could steal large numbers of votes.
Even optical scan machines have been shown to be vulnerable to
problems as simple as integer overflow attacks on their vote
counters~\cite{hurstiOSattack}.

An additional design challenge for e-voting machines is to ensure that
their security features survive the evolution of attacks over their
multidecadal operational lives.  Checkoway et~al.~\cite{avc-evt09}
illustrated this by using return-oriented programming~\cite{shacham2007geometry}, an
attack technique introduced in 2007, to defeat a hardware-based DEP
implementation in Sequoia AVC Advantage DREs designed during the 1980s.

In short, the vast majority of currently in-use electronic voting systems are 
significantly insecure, putting one of the most fundamental underpinnings of
democracy at risk: free elections. However, these systems (and their Internet 
counterparts) have come into use largely due to the enormous benefits derived
from their computerized nature. The question, then, is how can we keep the benefits
of electronic elections while also maintaining democratic integrity? 

